Coaxing Cosmic 21cm Fluctuations from the Polarized Sky using m-mode Analysis

In this paper we continue to develop the m-mode formalism, a technique for efficient and optimal analysis of wide-field transit radio telescopes, targeted at 21 cm cosmology. We extend this formalism to give an accurate treatment of the polarised sky, fully accounting for the effects of polarisation leakage and cross-polarisation. We use the geometry of the measured set of visibilities to project down to pure temperature modes on the sky, serving as a significant compression, and an effective first filter of polarised contaminants. We use the m-mode formalism with the Karhunen-Loeve transform to give a highly efficient method for foreground cleaning, and demonstrate its success in cleaning realistic polarised skies observed with an instrument suffering from substantial off axis polarisation leakage. We develop an optimal quadratic estimator in the m-mode formalism, which can be efficiently calculated using a Monte-Carlo technique. This is used to assess the implications of foreground removal for power spectrum constraints where we find that our method can clean foregrounds well below the foreground wedge, rendering only scales $k_\parallel < 0.02 h \,\mathrm{Mpc}^{-1}$ inaccessible. As this approach assumes perfect knowledge of the telescope, we perform a conservative test of how essential this is by simulating and analysing datasets with deviations about our assumed telescope. Assuming no other techniques to mitigate bias are applied, we recover unbiased power spectra when the per-feed beam width to be measured to 0.1%, and amplifier gains to be known to 1% within each minute. Finally, as an example application, we extend our forecasts to a wideband 400-800 MHz cosmological observation and consider the implications for probing dark energy, finding a medium-sized cylinder telescope improves the DETF Figure of Merit by around 70% over Planck and Stage II experiments alone.

==> formalism.tex <==
%!TEX root = paper.tex

\section{Formalism}

\label{sec:unpolarised}

\subsection{Unpolarised Case}

%% Cite Albert

Any transit telescope can be viewed as a collection of feeds, fixed relative to
the ground frame, where any particular feed $F_i$ measures a combination of the
electric field $E_a(\vnhat)$ coming from various directions on the
sky. Initially it will be instructive to pretend that the electric field is a
scalar quantity, allowing us to leave the complexity of the polarised notation
behind. The signal measured at a particular feed is given by
\begin{equation}
F_i = \int d^2\vnhat \, A_i(\vnhat) E(\vnhat) e^{2 \pi i \vnhat\cdot\vu_i}\; ,
\end{equation}
where the function $A_i(\vnhat)$ gives the amplitude of the response in that
direction, the exponential factor keeps track of the phase relative to an
arbitrary reference point, and $\vu_i$ is the displacement to that point,
divided by the wavelength. We assume that the radiation from the sky is
\emph{incoherent}, that is
\begin{equation}
\la E(\vnhat) E^* (\vnhat') \ra = \delta(\vnhat - \vnhat') I(\vnhat) \; .
\end{equation}

In traditional interferometry a visibility $\tvis_{ij}$ is the correlation
between two feeds $F_i$ and $F_j$ at a particular instant
\begin{align}
  \tvis_{ij} & = \la F_i F_j^* \ra \\
  &= \int d^2\vnhat \, A_i(\vnhat) A_j^*(\vnhat) e^{2 \pi i \vnhat \cdot \vu_{ij}}
  I(\vnhat)
\end{align}
where $\vu_{ij} = \vu_i - \vu_j$, the separation in the UV plane (fixed relative
to the ground). However where we are concerned with observing continuous fields
it will be more convenient to rescale this definition, and use a quantity
\begin{align}
\label{eq:nvis}
\vis_{ij} & = \frac{\nu^2}{2 k_b c^2 \Omega_{ij}} \tvis_{ij} \\ 
&= \frac{1}{\Omega_{ij}}\int d^2\vnhat \, A_i(\vnhat) A_j^*(\vnhat)
  e^{2 \pi i \vnhat \cdot \vu_{ij}} T(\vnhat)
\end{align}
where we have switched to using the brightness temperature $T$ instead of the
intensity $I = 2 k_b \nu^2 T / c^2$ (in the Rayleigh-Jeans limit). The quantity
$\Omega_{ij} = \sqrt{\Omega_i \Omega_j}$ is the geometric mean of the individual
beam solid angles
\begin{equation}
\Omega_i = \int \lv A_i(\vnhat) \rv^2 d^2\vnhat
\end{equation}
which also gives the effective antenna area $A_\text{eff} \Omega =
\lambda^2$. The usefulness of this definition of $\vis_{ij}$ is that our
visibilities are a temperature-like quantity whereas the usual quantity $\tvis$
is a flux --- specifically for a sky with uniform brightness temperature, with
our definition, the auto-correlation of an antenna $\vis_{ii} = T$.

These visibilities are sensitive to localised regions of the sky and so as the
Earth rotates their measured values change, we take this into account by
explicitly including the dependence on the azimuthal angle $\phi$. As the
Earths rotation ensures that the sky signal is periodic we can identify each
sidereal day of observation as equivalent and average over them. The measured
visibilities are also corrupted by instrumental noise, which we must
explicitly take account of by adding a noise term $n_{ij}(\phi)$
\footnote{Unlike the sky, the instrumental noise is not strictly periodic in
$\phi$, however, provided it is stationary we can treat it as such when
combining the measured sidereal days.}. We will write \cref{eq:nvis} in terms
of a transfer function $B_{ij}$ leaving the measured visibility as
\begin{equation}
  V_{ij}(\phi) = \int \! d^2\vnhat\, B_{ij}(\vnhat; \phi) T(\vnhat) + n_{ij}(\phi)
\end{equation}
where the transfer function is
\begin{equation}
  B_{ij}(\vnhat; \phi) = \frac{1}{\Omega_{ij}}A_i(\vnhat; \phi) A_j^*(\vnhat;
  \phi) e^{2 \pi i \vnhat \cdot\vu_{ij}(\phi)} \; .
\end{equation}
As expected in the rotating system the $UV$-plane changes orientation with
respect to the celestial sphere. Given the periodicity of the system, Fourier
transforming the system is an obvious next step
\begin{align}
  V^{ij}_m &= \int \frac{d\phi}{2\pi} V_{ij}(\phi) e^{-i m \phi} \\
  & = \sum_{l m'}\int \frac{d\phi}{2\pi} B^{ij}_{l m'}(\phi) a^{T*}_{l m'}
  e^{-i m \phi}+ n^{ij}_m
\end{align}
where to proceed to the second line we have inserted the spherical harmonic
expansions of both the sky, and the beam transfer function
\begin{align}
T(\vnhat) & = \sum_{lm} a^T_{lm} Y_{lm}(\vnhat) \; , \\
B_{ij}(\vnhat; \phi) & = \sum_{lm} B_{ij,lm}(\phi) Y_{lm}^*(\vnhat) \; .
\end{align}
Note that we have defined $B^{ij}_{lm}$ relative to the conjugate spherical
harmonic in order to simplify later notation. As the $\phi$ dependence simply
rotates the functions about the polar axis the transfer function is trivially
$B^{ij}_{lm}(\phi) = B^{{ij}}_{lm}(\phi\!=\!0) e^{i m \phi}$. %%Check me
Combined with the exponential factor in the integral, this simply generates
the Kroenecker delta $\delta_{mm'}$, and we find
\begin{equation}
\label{eq:vis_unpol1}
V^{ij}_m = \sum_{l} B^{ij}_{l m} a^{T}_{l m}+ n^{ij}_m \; .
\end{equation}



Calculation of the $B^\alpha_{l m}$ is performed by generating Healpix
\cite{HEALPIX} maps for every baseline at each frequency and performing the
Spherical Harmonic Transform (SHT).



\subsection{Matrix Notation}

The beam transfer matrices above can be written in an explicit matrix notation.
\begin{equation}
\left(\mB_m\right)_{(\alpha \nu) (l \nu')} = B_{\alpha;lm} \delta_{\nu \nu'}
\end{equation}
where the row index labels all baseline ($\alpha$) and frequency combinations
($\nu$), whereas the column index is over all multipole ($l$) and frequencies
($\nu'$). From here onwards we'll drop the subscript $m$, denoting the spherical
harmonic order, all the equations below are valid for any $m$.

The number of distinct baselines $n_\alpha$ is different to the maximum
multipole sampled $l_\tmax$, and usually $l_\tmax \ll n_\alpha$. The matrix
$\mB$ is of size $m \times n$, where $m = n_\alpha n_\nu$, $n = l_\tmax n_\nu$
and $n_\nu$ is the number of frequency bins. The sky, which we'll write as a
vector $\va$ of length $n$, is projected onto the space
of visibilities $\vv$ (vector length $m$)
\begin{equation}
\label{eq:matnot}
\vv = \mB\, \va^* + \vn \; .
\end{equation}

\subsection{Map making}

In astronomy being able to transform our measured signal into an accurate map
of the sky is essential. Whilst in this paper we explicitly avoid this process
for our analysis, preferring to carry it out directly in the data space, maps
are still needed for visualisation and cross-checking. Map-making with
interferometric data is generally a complicated process, usually performed
with algorithms such as CLEAN \tcite{CLEAN}. However, in our set up the
map-making process is conceptually simple.

First, we assume that the instrumental noise $\vn$ follows a complex gaussian
distribution with covariance $\mN$ (see \cref{app:noise}), and the
different frequency channels are independent. For stationary noise, the
$m$-modes are uncorrelated and the likelihood function of the observed sky for
a single $m$ and frequency $\nu$ is
\begin{equation}
\label{eq:like1}
p(\vv \vert \va) = \frac{1}{\lv \pi \mN \rv} \exp{\lp - \lp\vv - \mB\va\rp^\hconj \mN^{-1} \lp \vv - \mB \va \rp \rp}
\end{equation}
where the vector $\va$ contains all harmonic coefficients for the given $m$.

To estimate the sky corresponding to a given set of visibilities we will look
for a maximum likelihood solution $d p / d \va = 0$. In particularly we want
to find the value of $\va$ the minimises
\begin{equation}
\chi^2 = \lv \mN^{-\frac{1}{2}} \vv - \lp \mN^{-\frac{1}{2}} \mB \rp \va \rv^2 \; .
\end{equation}
The matrix $\mN^{-\frac{1}{2}}$ represents any factorisation such that
$(\mN^{-\frac{1}{2}})^\hconj \mN^{-\frac{1}{2}} = \mN^{-1}$. Provided $\mN$
contains no noiseless modes, it is positive-definite and so this factorisation
should exist. This could be found either a Cholesky or eigenvalue
decomposition. Depending on the number of baselines measured and the maximum
$l$ we are sensitive to, the problem may either be over- or under-constrained.
In either regime a solution can be found using the Moore-Penrose pseudo-inverse,
which in the latter case selects the solution which also minimises
$\lv\hat{\va}\rv^2$, effectively setting unconstrained degrees of freedom to 
zero\footnote{For details see \url{http://en.wikipedia.org/wiki/Moore-Penrose_pseudoinverse}}.
This leaves our best estimate of $\va$ as
\begin{equation}
\hat{\va} = \lp \mN^{-\frac{1}{2}} \mB \rp^+ \mN^{-\frac{1}{2}} \vv \; ,
\end{equation}
where the superscript $+$ denotes the pseudo-inverse. As both distinct
frequencies and $m$-modes are independent, map-making for a set of full sky
observations is a case of collating the estimates for each individual $\nu$
and $m$.

